EHRNoteQA: An LLM Benchmark for Real-World Clinical Practice Using Discharge Summaries

Discharge summaries in Electronic Health Records (EHRs) are crucial for clinical decision-making, but their length and complexity make information extraction challenging, especially when dealing with accumulated summaries across multiple patient admissions. Large Language Models (LLMs) show promise in addressing this challenge by efficiently analyzing vast and complex data. Existing benchmarks, however, fall short in properly evaluating LLMs' capabilities in this context, as they typically focus on single-note information or limited topics, failing to reflect the real-world inquiries required by clinicians. To bridge this gap, we introduce EHRNoteQA, a novel benchmark built on the MIMIC-IV EHR, comprising 962 different QA pairs each linked to distinct patients' discharge summaries. Every QA pair is initially generated using GPT-4 and then manually reviewed and refined by three clinicians to ensure clinical relevance. EHRNoteQA includes questions that require information across multiple discharge summaries and covers eight diverse topics, mirroring the complexity and diversity of real clinical inquiries. We offer EHRNoteQA in two formats: open-ended and multi-choice question answering, and propose a reliable evaluation method for each. We evaluate 27 LLMs using EHRNoteQA and examine various factors affecting the model performance (e.g., the length and number of discharge summaries). Furthermore, to validate EHRNoteQA as a reliable proxy for expert evaluations in clinical practice, we measure the correlation between the LLM performance on EHRNoteQA, and the LLM performance manually evaluated by clinicians. Results show that LLM performance on EHRNoteQA have higher correlation with clinician-evaluated performance (Spearman: 0.78, Kendall: 0.62) compared to other benchmarks, demonstrating its practical relevance in evaluating LLMs in clinical settings.

==> toc/checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes See Section \ref{1}
  \item Did you describe the limitations of your work?
    \answerYes See Section \ref{5}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{} Our dataset is derived from the MIMIC-IV database, which contains de-identified patient records from PhysioNet. For our study, we ensured compliance with data usage regulations by conducting experiments using Azure's HIPAA-compliant platform for running GPT models.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes See Appendices \ref{B}, \ref{E}, and \ref{F}. The full data will be provided by the link (which will be deprecated after review) in the Supplementary Materials. We will also release our experimental code through Github.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes See Appendices \ref{B.2} and \ref{E.1}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes See Appendix \ref{E.1}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes See Appendix \ref{B.2}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes See Section \ref{3} and \ref{4}
  \item Did you mention the license of the assets?
    \answerYes See Appendix \ref{B}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes The full data will be provided by the link (which will be deprecated after review) in the Supplementary Materials.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes See Section \ref{4.1} and \ref{4.3}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{} Our dataset is derived from the MIMIC-IV database, which contains de-identified patient records from PhysioNet. Thus, our dataset does not include any personally identifiable information or offensive content.
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes See Appendices \ref{C.3} and \ref{F.2}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNo{}  The dataset we used, MIMIC-IV, has been approved by the Institutional Review Boards of both Beth Israel Deaconess Medical Center (Boston, MA), and the Massachusetts Institute of Technology (Cambridge, MA).
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
